USBCaptchaIn: Preventing (Un)Conventional Attacks from Promiscuously Used USB Devices in Industrial Control Systems

Industrial Control Systems (ICS) are sensible targets for high profile attackers and advanced persistent threats, which are known to exploit USB thumb drives as an effective spreading vector. In ICSes, thumb drives are widely used to transfer files among disconnected systems and represent a serious security risks, since, they may be promiscuously used in both critical and regular systems. The threats come both from malware hidden in files stored in the thumb drives and from BadUSB attacks [16]. BadUSB leverages the modification of firmware of USB devices in order to mimic the behaviour of a keyboard and send malicious commands to the host. We present a solution that allows a promiscuous use of USB thumbs drives while protecting critical machines from malware, that spread by regular file infection or by firmware infection. The main component of the architecture we propose is an hardware, called USBCaptchaIn, intended to be in the middle between a critical machine and all USB devices. We do not require users to change the way they use thumb drives. To avoid human-errors, we do not require users to take any decision. The proposed approach is highly compatible with already deployed products of a ICS environment and proactively blocks malware before they reach their targets. We describe our solution, provide a thorough analysis of the security of our approach in the ICS context, and report the informal feedback of some experts regarding our first prototypes.

==> 101-acontext.tex <==
\section{Context - NOTE}


In our approach, we consider as a machines both personal netbooks and embedded systems (e.g. PLCs).
We assume to have two different type o machines, critical and non-critical. Non-critical machines are those machines potentially malicious and possible sources of attack vectors against critical machines.
%
We assume each critical machine equipped with \U\ and all USB devices, both storage and USB HIDs, are connected to critical machines through it.

Our purpose is to protect critical machines against two main type of malware. The firs type are the one spread as malicious software which leverage USB storage to infect machines. They can be executable files or embedded into readable files, e.g. javascript object inserted in pdf file or malicious macros of MS word. The second type are the ones spread through malicious firmware that present themself as data storage but act as malicious HIDs. 


==> 104-threatmodel.tex <==
\section{Threat Model}

%In our model threats can be generated in non-critical realm and spread over critical realm by means of reading operation of RSD containing malware or file embedding malicious code. 
%Further, Keyboard or mice containing malicious 


In our model non-critical realm, and malicious RSDs are potentially sources of attacks.
Threats are mainly represented by injection of malicious code in files stored in a RSD, the tampering of any data stored in it, and any input provided by malicious RSDs. Note that, both embedding malicious code to any file or tampering with any kind of data are considered equally illegal.
We consider an attack every write operation performed by a regular machine on something that is supposed to be read by a critical machine, as well as, changes performed by regular machines to metadata or directory structures. 


%For instance, consider the case in which a control logic stored in an RSD is destined for deployment. An attacker 
%might want to force the use of an older version that is known to contain some bugs, and restoration of a full volume to a previous version can pass unnoticed.







